Laser assisted electron dynamics

We apply the convergent close-coupling (CCC) formalism to analyse the processes of laser assisted electron impact ionisation of He, and the attosecond time delay in the photodetachment of the H^{-} ion and the photoionisation of He. Such time dependent atomic collision processes are of considerable interest as experimental measurements on the relevant timescale (attoseconds 10^{-18} s) are now possible utilising ultrafast and intense laser pulses. These processes in particular are furthermore of interest as they are strongly influenced by many-electron correlations. In such cases their theoretical description requires a more comprehensive treatment than that offered by first order perturbation theory. We apply such a treatment through the use of the CCC formalism which involves the complete numeric solution of the integral Lippmann-Schwinger equations pertaining to a particular scattering event. For laser assisted electron impact ionisation of He such a treatment is of a considerably greater accuracy than the majority of previous theoretical descriptions applied to this problem which treat the field-free scattering event within the first Born approximation. For the photodetachment of H^{-} and photoionisation of He, the CCC approach allows for accurate calculation of the attosecond time delay and comparison with the companion processes of photoelectron scattering on H and He^{+}, respectively.

==> Plots/ExamplePlot <==
file="Factor8Comp"

set terminal epslatex 8 newstyle color standalone header \
   "\\usepackage[T1]{fontenc}\n\\usepackage{lmodern}\n\\usepackage{amsmath}\n\\usepackage{amssymb}\n"

set output file.'.tex'

set lmargin at screen 0.15
set rmargin at screen 0.95

TOP=0.8
DY=0.3

set offset 0.05, 0.05

set ylabel 'TDCS a.u.' offset 0,-5

set style line 1 lw 3 lt rgb "blue"
set style line 2 lw 3 lt rgb "red"
set style line 3 lw 3 lt rgb "green"
set style line 4 lw 3 lt rgb "purple"
set style line 5 lw 3 lt rgb "orange"

set xrange [-200:200]
#set xtics 30
set multiplot layout 2,1

set xtics 30
set format x ''
set format y '%.1f'

set tmargin at screen TOP
set bmargin at screen TOP-1*DY
set yrange [0:2.0]
set ytics 0.0,0.4,2.0
plot "/home/573/awb573/HonoursProject/1keV/1000.0000000eV/TDCS/ta_10_5" u 1:($2*27.2/(5.29E-9)**2) w l ls 1 t 'ta\_10\_5', \
"/home/573/awb573/HonoursProject/1keV/1000.0000000eV/TDCS/ta_10_10" u 1:($2*27.2*8/(5.29E-9)**2) w l ls 2 t '8*ta\_10\_10'#, \

set xlabel '$\phi_b$'
set format x '%g'

set tmargin at screen TOP-1*DY
set bmargin at screen TOP-2*DY
set yrange [0:2.5]
set ytics 0.0,0.4,2.2
set ylabel ''
plot "/home/573/awb573/HonoursProject/1keV/1000.0000000eVBorn/TDCS/ta_10_5" u 1:($2) w l ls 1 t 'Born ta\_10\_5', \
"/home/573/awb573/HonoursProject/1keV/1000.0000000eVBorn/TDCS/ta_10_10" u 1:($2*8) w l ls 2 t '8*Born ta\_10\_10'#, \
#"/home/573/awb573/HonoursProject/Plots/datathief.txt" u 1:($2) w lp ls 1 title "FF 7-12eV 0.7-1.0au"

unset multiplot

set output # finish the current output file

system(sprintf('latex %s.tex && dvips %s.dvi && ps2pdf %s.ps',file,file,file))
system(sprintf('rm %s.tex %s.dvi %s.aux %s.log %s-inc.eps',file,file,file,file,file))


==> Plots/plotMomentumTrans <==
file="Momentum"

set terminal epslatex 12 newstyle color standalone header \
   "\\usepackage[T1]{fontenc}\n\\usepackage{lmodern}\n\\usepackage{amsmath}\n\\usepackage{amssymb}\n"

set output file.'.tex'

set style line 1 lw 3 lt 1 lc rgb "blue"
set style line 2 lw 3 lt 2 lc rgb "red"
set style line 3 lw 3 lt rgb "green"
set style line 4 lw 3 lt rgb "purple"
set style line 5 lw 3 lt rgb "orange"

m=1

p(E)=sqrt((E+m*137**2)**2-m**2*137**4)/137
q(E)=sqrt(2*m*E)

set xrange [1:1E8]
#set yrange [0:100]

set logscale x
set logscale y

set xtics format "$10^{%T}$"
set ytics format '$10^{\scriptscriptstyle %+T}$'

set xlabel "Energy (eV)"
set ylabel "Momentum (a.u.)" offset 2,0

plot q(x/27.211) ls 2 title "classical $p$", p(x/27.211) ls 1 title "relitavistic $p$" 

set output # finish the current output file

system(sprintf('latex %s.tex && dvips %s.dvi && ps2pdf %s.ps',file,file,file))
system(sprintf('rm %s.tex %s.dvi %s.aux %s.log %s-inc.eps',file,file,file,file,file))

file="MomentumTrans"

set terminal epslatex 12 newstyle color standalone header \
   "\\usepackage[T1]{fontenc}\n\\usepackage{lmodern}\n\\usepackage{amsmath}\n\\usepackage{amssymb}\n"

set output file.'.tex'

set style line 1 lw 3 lt rgb "blue"
set style line 2 lw 3 lt rgb "red"
set style line 3 lw 3 lt rgb "green"
set style line 4 lw 3 lt rgb "purple"
set style line 5 lw 3 lt rgb "orange"

set angles degrees

m=1

p(E)=sqrt(2*m*E)

q(Ei,Ef,theta)=sqrt( (p(Ei))**2+(p(Ef))**2-2*p(Ei)*p(Ef)*cos(theta))

unset logscale x
unset logscale y

set xlabel "Scattered angle $\\phi_a$ (Degrees)"
set ylabel "Momentum Transfer $q$ (a.u.)" offset 0,0

set xrange [0:180]

set xtics format '%0.f'
set ytics format '%0.f'

set mxtics 4
set mytics 4

plot q(1000/27.211,(1000-24.58741 - 10)/27.211,x) ls 1 not "Momentum Transfer $q$" 

set output # finish the current output file

system(sprintf('latex %s.tex && dvips %s.dvi && ps2pdf %s.ps',file,file,file))
system(sprintf('rm %s.tex %s.dvi %s.aux %s.log %s-inc.eps',file,file,file,file,file))

